Conceptual Design of BabyIAXO, the intermediate stage towards the International Axion Observatory

This article describes BabyIAXO, an intermediate experimental stage of the International Axion Observatory (IAXO), proposed to be sited at DESY. IAXO is a large-scale axion helioscope that will look for axions and axion-like particles (ALPs), produced in the Sun, with unprecedented sensitivity. BabyIAXO is conceived to test all IAXO subsystems (magnet, optics and detectors) at a relevant scale for the final system and thus serve as prototype for IAXO, but at the same time as a fully-fledged helioscope with relevant physics reach itself, and with potential for discovery. The BabyIAXO magnet will feature two 10 m long, 70 cm diameter bores, and will host two detection lines (optics and detector) of dimensions similar to the final ones foreseen for IAXO. BabyIAXO will detect or reject solar axions or ALPs with axion-photon couplings down to $g_{a\gamma} \sim 1.5 \times 10^{-11}$ GeV$^{-1}$, and masses up to $m_a\sim 0.25$ eV. BabyIAXO will offer additional opportunities for axion research in view of IAXO, like the development of precision x-ray detectors to identify particular spectral features in the solar axion spectrum, and the implementation of radiofrequency-cavity-based axion dark matter setups.

==> sections/BabyIAXO_soft.tex <==


A collaboration-wide working group has been established to deploy common software tools to be made available to the collaboration members, giving access to the experimental data generated during the BabyIAXO data taking phase. These tools will be combined and used during the data production, processing, analysis and storage. REST\,\cite{Castel:2018gcp,Galan:2019ake} a data analysis framework based on ROOT, will be used to interface and/or build those tools. Data production will be linked to the versioning system and metadata description of REST to assure full traceability of the data processing.

The IAXO software tools will allow to address issues related to the following points.

\begin{itemize}
\item {\bf Axion signal generation}. It will allow to produce a Monte Carlo image of the expected axion signal on babyIAXO detectors, after including different contributions to the signal response, as it is an accurate description of the solar axion flux, the axion-photon oscillations on an arbitrary magnetic field map, optics response, etc.

\item {\bf Monte Carlo background model}. Matter-radiation physics packages will be interfaced with the data analysis framework to provide proper Monte Carlo detector data. Detector groups will be able to assess the impact and contribution of different contaminations on their detector setup, in view of optimizing a common detector shielding for the detection platform.

\item {\bf Detector data analysis}. Detector background and tracking data analysis will be performed with REST, providing a common tool to access and to store the data which will be properly tagged, classified and merged with other babyIAXO experimental setup variables.

\item {\bf Experimental sensitivity}. Axion signal generation, Monte Carlo background models and experimental detector data will be appropriately combined into a statistics package providing tools to determine the axion couplings to ordinary matter from both, the collected experimental data or Monte Carlo generated data.

\item {\bf Visualization and data access}. Any resulting event data and experiment data generated will be visualized and accessible by means of an internal web interface. Access performance will be optimized by means of indexing REST metadata structures into a centralized SQL database.

\end{itemize}


%In addition to software infrastructure, first discussions on the needed computing infrastructure are ongoing. BabyIAXO computing will have to satisfy the needs of: 1) experimental data storage, 2) background simulation data storage, 3) slow control data storage (data base), 4) data analysis computations, 5) signal and background simulation computation. Due to the low counting rate of the detectors, the computing needs are expected to be relatively modest.

\subsubsection{Open Research Data Management Plan}

The collaboration has started discussion on a Data Management Plan that contemplates the release of research data to the scientific community. Partly funded by the European Research Council (ERC), the collaboration is encouraged to participate in the Open Research Data Pilot Program of this institution. The current intentions of the collaboration in this respect include:
\begin{itemize}
   \item Properly organize and identify the main research data sets produced by BabyIAXO.
   \item Release and maintain them in open repositories, within a reasonable time after their production and after the main related publications by the collaboration. 
   \item Append all necessary metadata to assure traceability of pre-processed data. Use well established data formats and documented protocols.
   \item Produce and maintain adequate documentation and software tools and interfaces to browse the released data by external end-users. 
\end{itemize}
Additional details of the implementation of these measures will be produced at more advanced stages of the project.
